Developments in entanglement theory and applications to relevant physical systems

This Thesis is devoted to the analysis of entanglement in relevant physical systems. Entanglement is the conducting theme of this research, though I do not dedicate to a single topic, but consider a wide scope of physical situations. I have followed mainly three lines of research for this Thesis, with a series of different works each, which are, Entanglement and Relativistic Quantum Theory, Continuous-variable entanglement, and Multipartite entanglement.

==> DEA0.tex <==
%%% Thesis Introduction --------------------------------------------------
%\renewcommand{\MakeUppercase}{}
%\nonumchapter{Introduction}
\chapter{Introduction}
\pagestyle{fancy}
%\CHAPTER{Introduction}

\section{Overview and motivation}

Quantum computation and quantum information is the field that deals
with the information processing and transmission making use of
quantum systems. This is a discipline that has begun its development
in recent years, and to which a lot of effort is being devoted (for
a review of the field, see for example \cite{GM02,nielsen}). Its
interest stems from the fact that there are physical tasks regarding
information processing and transmission that can be possibly done
more efficiently with quantum systems than with the ordinary
classical ones. Some examples are the following:

\begin{enumerate}
\item Regarding information processing we highlight
\begin{itemize}
    \item \textbf{The factorization of large integer numbers into primes\cite{S97}.}

    This takes a time that grows as $\exp(N)$ in the number of digits $N$ of the integer being
factorized with the most powerful classical algorithms known. That
is the property in which many classical cryptography systems are
based, i.e. public key distribution. With Shor's algorithm a quantum
computer would only use a polynomial time in $N$.

    \item \textbf{Search algorithms \cite{G97}.}

    ``Quantum mechanics helps in searching for a needle in a haystack" (L. Grover).
    With a classical computer it takes a time of order $N$ to find a
    given item in a disorganized list of size $N$. In a quantum computer it would take
a time that grows as $\sqrt{N}$, with Grover's algorithm.

   \end{itemize}

\item Regarding information transmission, we mention
\begin{itemize}
    \item \textbf{Quantum cryptography \cite{crypto1,crypto2}.}

    The private distribution of secure keys, for use in
    cryptography, is a reality. Nowadays there are some companies
    which offer this service. This feature relies in the
    impossibility of distinguishing with certainty two
    non-orthogonal quantum states.

    \item \textbf{Dense coding \cite{BW92}.}

     With quantum mechanics
     it is possible to transmit two bits of
    information with a single quantum bit, in a secure way.

    \item \textbf{Quantum teleportation \cite{tele1,BBM+98,tele2}.}

    This is a feature very useful in quantum information. It is a procedure to move
    quantum states around without making use of a communication
    channel. With this protocol a copy of a certain quantum state is
    obtained in another specified place. This implies the
    destruction of the initial state, because the cloning of quantum states is forbidden by quantum
    linearity (no-cloning theorem).

\end{itemize}

\end{enumerate}

Some of the previous applications make use of a genuine quantum
resource, namely \textbf{Entanglement}. In the early days of
quantum mechanics, Erwin Schr\"{o}dinger already realized the
importance of this quantum property. He said, ``Entanglement is
the characteristic trait of Quantum Mechanics". Roughly speaking,
entanglement are genuine quantum correlations between spatially
separated physical systems. To show the difference between these
non-local, quantum correlations and purely classical ones, we
consider an example conceived by Asher Peres \cite{P78,P95}:
Suppose a bomb, initially at rest, which explodes into two
fragments carrying opposite momenta $\mathbf{J}_1$,
$\mathbf{J}_2=-\mathbf{J}_1$ (see FIG. \ref{figint1}). An observer
measures the magnitude
$\mathrm{sign}(\hat{\alpha}\cdot\mathbf{J}_1)$, where
$\hat{\alpha}$ is a unit vector with a fixed arbitrary direction.
The result of the measurement, called a, is $+1$ or $-1$.
Additionally, a second observer measures
$\mathrm{sign}(\hat{\beta}\cdot\mathbf{J}_2)$, where $\hat{\beta}$
is another unit vector with another fixed arbitrary direction. The
result can only be $b=\pm 1$.

\begin{figure}[t]
\begin{center}
\includegraphics{peres3.eps}
\end{center}
\caption{Schematic experiment in which a bomb, initially at rest,
explodes into two fragments with opposite momenta,
$\mathbf{J}_2=-\mathbf{J}_1$.\label{figint1}}
\end{figure}

The experiment is repeated $N$ times. We call $a_j$ and $b_j$ the
results measured by these observers for the $j$th bomb. If the
observers compare their results, they find a correlation
\begin{equation}
\langle ab \rangle=\sum_j a_j b_j/N.\nonumber
\end{equation}
For example, if $\hat{\alpha}=\hat{\beta}$, they obtain $\langle
ab \rangle=-1$.

To compute $\langle ab \rangle$ for arbitrary $\hat{\alpha}$ and
$\hat{\beta}$, we consider the sphere shown in FIG. \ref{figint2}.
The plane orthogonal to $\hat{\alpha}$ divides the sphere in two
hemispheres. We have $a=1$ if $\mathbf{J}_1$ points through one of
these hemispheres and $a=-1$ if it points through the other
hemisphere. Similarly, the regions where $b=\pm 1$ are limited by
the intersection of the sphere with the plane orthogonal to
$\hat{\beta}$. This way, the sphere is divided into four sections,
as shown in FIG. \ref{figint2}. The shaded sections have $\langle ab
\rangle=1$, while the unshaded ones have $\langle ab \rangle=-1$.
The classical correlation for uniformly distributed $\mathbf{J}_1$
results
\begin{equation}
\langle ab
\rangle=[\theta-(\pi-\theta)]/\pi=-1+2\theta/\pi.\label{formperes1}
\end{equation}
\begin{figure}[t]
\begin{center}
\includegraphics{peres1def.eps}
\end{center}
\caption{Auxiliary figure for computing the classical correlation
(\ref{formperes1}). The shaded areas correspond to $\langle
ab\rangle=1$, while the unshaded ones correspond to $\langle
ab\rangle=-1$.\label{figint2}}
\end{figure}
Regarding now the quantum mechanical case, we consider two
spatially separated spin $1/2$ particles $1$ and $2$ in the
singlet state
\begin{equation}
|\Psi\rangle=\frac{1}{\sqrt{2}}(|\uparrow_1\downarrow_2\rangle-|\downarrow_1\uparrow_2\rangle),\nonumber
\end{equation}
where the arrows denote the third component of spin along an
arbitrary direction. An observer measures the observable
$\hat{\alpha}\cdot\vec{\sigma}_1$, while another one measures
$\hat{\beta}\cdot\vec{\sigma}_2$, being $\vec{\sigma}_1$ and
$\vec{\sigma}_2$ the Pauli spin matrices associated to particles
$1$ and $2$ respectively. $\hat{\alpha}$ and $\hat{\beta}$ are
arbitrary unit vectors. We denote as before $a$ and $b$ the
results of these measures, taking values $\pm 1$. It can be shown
that in this case, the correlation is
\begin{equation}
\langle
ab\rangle=-\hat{\alpha}\cdot\hat{\beta}=-\cos\theta.\label{formperes2}
\end{equation}
We plot (\ref{formperes1}) and (\ref{formperes2}) in FIG.
\ref{figint3}. This figure shows how the quantum correlation is
always stronger than the classical one, except where both are $0$
or $\pm 1$. This qualitatively different behavior of the quantum
and classical correlations has very profound implications, as John
Bell shown \cite{Bell64}: realism+locality is incompatible with
quantum mechanics.

\begin{figure}
\begin{center}
\includegraphics{peres2def.eps}
\end{center}
\caption{Quantum correlation (\ref{formperes2}) (solid) and
classical one (\ref{formperes1}) (dashed), $\langle ab\rangle$, as
functions of $\theta$.\label{figint3}}
\end{figure}

At the same time that the field of quantum information and
computation evolves, more and more evidence appears that shows the
crucial role of entanglement in this field.
 Bipartite and multipartite entanglement is one of the features
that give rise to many of the developments of quantum computation
and information, like quantum cryptography \cite{crypto1,Eke91},
dense coding \cite{BW92}, quantum teleportation
\cite{tele1,BBM+98,tele2} and aspects of quantum computation
\cite{nielsen}, among others. A lot of effort is being devoted to
obtain separability criteria (to decide whether a given mixed or
pure state is entangled or not), and to measure and characterize
entanglement. For a review, see \cite{LBC+00}. The evaluation of the
entanglement of a composite state is thus a main task to be done.

While multipartite entanglement and mixed states entanglement are
resulting very difficult to study theoretically, entanglement of
pure states of systems with just two components is much better known
and very interesting for applications
\cite{Eke91,BW92,tele1,BBM+98,tele2}. The Schmidt
decomposition\index{Schmidt decomposition}
\cite{schmidtdisc1,schmidtdisc2} is a valuable tool for analyzing
these states entanglement. This procedure (not to be confused with
the Gram-Schmidt orthogonalization procedure, which is a different
one) relies on the singular value decomposition of a square matrix
\cite{nielsen}. It allows to express an arbitrary pure bipartite
state as `sum of diagonal biorthogonal products'. This way the
entanglement of this state is easily evaluated and ready to use. In
Appendix \ref{appendB} we explain in detail the Schmidt
decomposition procedure, both for finite dimensional systems and for
those described by continuous variables.

In this work we obtain an alternative way \cite{lljl} to compute the
Schmidt decomposition\index{Schmidt decomposition} for systems
described with continuous variables, different to the usual one. It
has the advantage of preserving the analytical dependence of the
states, and it is well motivated due to the research community
concern in entanglement. We also study some specifical systems of
interest, using this method.

\section{Description of this work}

In this work we consider the case of continuous variables
entanglement. For us, these variables may be
$\{a+a^{\dag},i(a^{\dag}-a)\}$ which commute as phase space
variables do. We also refer to continuous variable entanglement in
systems described by momentum and/or energy observables. Precisely,
the entanglement of continuous variables stems from the original EPR
article \cite{epr}. The systems with continuous variables have been
studied thoroughly both theoretically and experimentally,
\cite{V94,FSB+98,LB99,G01,GEC+03,AB05} and references therein.
However, the treatment of the entanglement of systems with
continuous variables, from a practical point of view, is far from
straightforward. Until now, obtaining the Schmidt
decomposition\index{Schmidt decomposition} in the continuous case
required solving the corresponding integral equations
\cite{schmidtcont,eberly1,eberly2,eberly3,eberly4}. They had to be
discretized, losing the continuous dependence of the initial state.
Here we propose a method \cite{lljl} to perform the Schmidt
decomposition for this case, to the accuracy desired, keeping the
continuous character of the variables. This method consists of two
steps:

\begin{enumerate}

\item We decompose the bipartite system wave function, $f(p,q)$, by
using two denumerable and complete sets of orthonormal functions,
$\{O^{(1)}_n(p)\}$, $\{O^{(2)}_n(q)\}$, of $L^2$, in the form:
\begin{equation}
f(p,q)=\sum_{m,n}C_{mn}O^{(1)}_m(p)O^{(2)}_n(q).\label{eq11}
\end{equation}
The purpose of this step is to transform the continuous problem
into a discrete one (a necessary step for the numerical
computation), while preserving the continuous dependence of
$f(p,q)$.

\item Then we apply the (finite dimensional) Schmidt procedure to
(\ref{eq11}) in order to write the wave function $f(p,q)$ as
diagonal sum of biorthogonal terms:
\begin{equation}
f(p,q)=\sum_n
\sqrt{\lambda_n}\psi^{(1)}_n(p)\psi^{(2)}_n(q).\nonumber%\label{eq12}
\end{equation}
\end{enumerate}
 The orthonormal functions $\psi^{(1)}_n(p)$, $\psi^{(2)}_n(q)$ -the modes- will be
some particular linear combinations of $O^{(1)}_n(p)$,
$O^{(2)}_n(q)$, respectively. Notice that we are using the Schmidt
procedure for discrete systems to obtain the decomposition for the
continuous case. This is much more tractable, as it implies
diagonalizing matrices instead of solving integral equations.

The rationale for this procedure is the expectation that only a
few $O_n$ will suffice: A handful of appropriate orthonormal
functions will approximate $f(p,q)$ to the desired accuracy. We
finish by pointing out some properties of this method, namely

\begin{itemize}

\item We obtain complete analytic characterization of the modes
$\psi^{(1)}_n(p)$, $\psi^{(2)}_n(q)$ to the desired precision. Our
method surpasses the standard numerical procedures in that keeps the
continuous features present in $f(p,q)$.

\item We remark the portability of the attained modes
$\psi^{(1)}_n(p)$, $\psi^{(2)}_n(q)$ that are ready for later uses.

\item For the physical systems analyzed, we found that the number of
$O_n$ functions required is small. For example, in the biphoton case
analyzed in Chapter \ref{s4}, the accuracy (error) was of around
$2\%$ with $26\times 26$ $C_{mn}$ matrices. Considering the case of
two electrons which interact via QED, studied in detail in Chapter
\ref{qed}, the error was of $0.7\%$ with $12\times 12$ matrices.
\end{itemize}

In this work we begin with a detailed exposition of our procedure in
Chapter \ref{s2}.

In Chapter \ref{s4} we apply our method to a relevant case: the
entanglement of two photons created by parametric down-conversion.
We compare our results (leading to well known, continuous
functions) with those computed by standard numerical methods
\cite{eberly1} that produce sets of points: discrete functions.
Both procedures agree remarkably well.

In Chapter \ref{saf} we give additional formulas that may help to
apply our method in some situations. We also generalize the method
to pure states of bipartite systems with multiple continuous
variables (more than just two).

In Chapter \ref{qed} we study the Quantum Electrodynamics (QED)
interaction between two electrons, at lowest order. We observe how
the correlations in the momenta of the pair of electrons grow with
time, always preserving the antisymmetry of the state associated to
fermion statistics.

In Chapter \ref{unstable} we consider the final products of an
unstable system like an excited atom which emits a photon and decays
into the ground state, or a nucleus which radiates a particle
entangled with it. We analyze the entanglement in energies of these
final particles. We study its dependence on the decay width of the
system and on time. We observe that the entanglement grows with
time, whereas the wider the decay width, the lesser the
entanglement. We also compute the power-law corrections in $t$ to
the exponential decay, and obtain the entangled dependence in
energies of this corrections.

In Chapter \ref{delta} we decompose the Dirac delta, a case of
physical and mathematical interest.

In Appendix \ref{appendB} we review the Schmidt procedure for
expressing a general bipartite pure state as `diagonal sum of
biorthogonal products'. We describe the finite dimensional case
and the continuous case.

Finally, In Appendix \ref{appendA} we enumerate some of the
properties of a specific and widely used (in other contexts; see,
for example, \cite{LL05b}) type of denumerable orthonormal functions
$O^{(1)}_n(p)$, $O^{(2)}_n(q)$, namely: the orthogonal polynomials.
Throughout this work we consider natural units $\hbar=c=1$ unless
otherwise indicated.
%%% ----------------------------------------------------------------------


==> DEA6.tex <==
\def\baselinestretch{1}

%\nonumchapter{Conclusions}
\chapter{Conclusions}


\def\baselinestretch{1.66}


%%% ----------------------------------------------------------------------


In this work we introduce a method \cite{lljl} for computing the
Schmidt decomposition of bipartite pure states of systems with
continuous degrees of freedom. In the existing literature
\cite{schmidtcont,eberly1,eberly2,eberly3,eberly4} the
decomposition produced sets of points as approximation to the
modes. Our method gives linear combinations of the well known
orthonormal functions as approximation to them. When these
functions are chosen properly, a handful of them is enough to
reach the desired accuracy. We introduce some criteria for the
control of convergence and truncation error.

The result of our method for the decomposition of a biphoton state
produced by parametric down-conversion agrees with the numeric
results in the literature \cite{eberly1}.

 We give additional formulas for the calculation of the $C_{mn}$ coefficients
(\ref{eq25}) with derivatives instead of integrals. We generalize
our method to pure states of bipartite systems with multiple
continuous variables (more than just two).

 We analyze the QED
interaction between two electrons studying the entanglement in
momenta that appears as a result of it. We observe how as the
energy uncertainty gets lesser with time, and thus the total
energy becomes conserved, the correlations increase.

 We
investigate unstable systems that decay in a pair of entangled
particles. We study the energy entanglement dependence on the decay
width and on time, and we conclude that, while the entanglement in
energies grows with time (and eventually reaches a maximum) the
entanglement decreases with increasing width. We obtain the energy
correlations of the power-law corrections in $t$ to the exponential
decay.

 Finally, we describe the Dirac delta
case.
%%% ----------------------------------------------------------------------

